Developing emotion recognition for video conference software to support people with autism

We develop an emotion recognition software for the use with a video conference software for autistic individuals which are unable to recognize emotions properly. It can get an image out of the video stream, detect the emotion in it with the help of a neural network and display the prediction to the user. The network is trained on facial landmark features. The software is fully modular to support adaption to different video conference software, programming languages and implementations.

==> Aliases.tex <==
%
% texAbbrev.tex: Einige Abkürzugen 
%

\newcommand{\ia}{i.\,Allg.\ }
\newcommand{\dht}{d.\,h.\ }
\newcommand{\ua}{u.\,a.\ }
\newcommand{\so}{s.\,o.\ }
\newcommand{\zb}{z.\,B.\ }
\newcommand{\zbdp}{z.\,B.:\ }
\newcommand{\idr}{i.\,d.\,R.\ }
\newcommand{\zt}{z.\,T.\ } 
\newcommand{\zz}{z.\,Zt.\ } 
\newcommand{\igs}{i.\,Ggs.\ } 

\newcommand{\code}{\ttfamily}

\newcommand{\svs}{\vspace*{0.5ex}} 
\newcommand{\myrule}{\ \vspace{1ex} \\ \hrule} 
\newcommand{\figref}[1]{Abb.~\ref{#1}} 
\newcommand{\secref}[1]{Abschnitt~\ref{#1}} 
\newcommand{\mymargin}[1]{\marginpar{\raggedright \footnotesize \sffamily #1}} 

\definecolor{dkgreen}{rgb}{0.0, 0.2, 0.13}
\definecolor{mauve}{rgb}{0.69, 0.61, 0.85}

\lstdefinestyle{c}{
	belowcaptionskip=1\baselineskip,
	breaklines=true,
	frame=L,
	xleftmargin=\parindent,
	language=C,
	showstringspaces=false,
	basicstyle=\footnotesize\ttfamily,
	keywordstyle=\bfseries\color{green!40!black},
	commentstyle=\itshape\color{purple!40!black},
	identifierstyle=\color{blue},
	stringstyle=\color{orange},
	escapeinside=``,
	breaklines=true,
	postbreak=\mbox{\textcolor{red}{$\hookrightarrow$}\space},
	captionpos=b
}

\lstdefinestyle{bash}{
	language=bash,
	keywordstyle=\color{blue},
	commentstyle=\color{dkgreen},
	stringstyle=\color{mauve},
	numbers=left,
	basicstyle=\scriptsize\ttfamily,
	showspaces=false,
	frame=shadowbox,
	xleftmargin=0.5cm,
	escapeinside=``,
	breaklines=true,
	postbreak=\mbox{\textcolor{red}{$\hookrightarrow$}\space},
	captionpos=b
}

\renewcommand{\topfraction}{0.95}
\renewcommand{\bottomfraction}{0.95}

\newenvironment{trilist}{
    \renewcommand{\labelitemi}{\(\triangleright\)}
    \renewcommand{\labelitemii}{{\bfseries -}}
    \setlength{\partopsep}{0ex plus .5ex minus .5ex} 
    \setlength{\topsep}{-1ex plus .5ex minus .5ex} 
    \setlength{\parskip}{1.2ex plus .5ex minus .5ex}
    \setlength{\itemsep}{0pt plus .5ex minus .5ex}
    \setlength{\parsep}{0pt plus .5ex minus .5ex} 
    \begin{itemize}
    }
   {\end{itemize}}

\makeatletter

\renewcommand\listoftables{%
	\subsection{\listtablename}%
	\@starttoc{lot}%
}
\renewcommand\listoffigures{%
	\subsection{\listfigurename}%
	\@starttoc{lof}%
}

